Higher-Order Asynchronous Effects

We explore asynchronous programming with algebraic effects. We complement their conventional synchronous treatment by showing how to naturally also accommodate asynchrony within them, namely, by decoupling the execution of operation calls into signalling that an operation's implementation needs to be executed, and interrupting a running computation with the operation's result, to which the computation can react by installing interrupt handlers. We formalise these ideas in a small core calculus and demonstrate its flexibility using examples ranging from a multi-party web application, to pre-emptive multi-threading, to (cancellable) remote function calls, to a parallel variant of runners of algebraic effects. In addition, the paper is accompanied by a formalisation of the calculus's type safety proofs in Agda, and a prototype implementation in OCaml.

==> aeff.tex <==
% !TEX root = paper.tex

\lstdefinelanguage{aeff}{
    backgroundcolor=\color{white},
    basicstyle={\small\sffamily},
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    columns=fullflexible,
    commentstyle=\color{codegray},
    identifierstyle={\sffamily},
    keepspaces=true,
    keywordstyle=[1]{\color{keywordColor}},
    mathescape=true,
    numbers=none,
    numbersep=5pt,
    numberstyle=\tiny\color{codegray},
    rulecolor=\color{lightgray},
    sensitive=true,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    stringstyle=\color{codepurple},
    tabsize=2,
    texcl=true,
    xleftmargin=1em,
    xrightmargin=1em,
    morekeywords=[1]{
     and,
     any,
     as,
     await,
     bool,
     do,
     else,
     empty,
     end,
     external,
     fun,
     if,
     in,
     initially,
     kernel,
     kill,
     let,
     load,
     match,
     of,
     operation,
     process,
     promise,
     raise,
     rec,
     return,
     run,
     signal,
     spawn,
     string,
     then,
     try,
     to,
     type,
     unbox,
     unit,
     until,
     use,
     using,
     val,
     when,
     with,
     @
    },
    morecomment=[n]{(*}{*)},
    morestring=[b]",
    literate={->}{$\rightarrow\,$}{1}
    		{|->}{$\,\mapsto\,$}{1}
                {;}{$\boldsymbol;$}{1}
                {<<}{$\langle$}{1}
                {>>}{$\rangle$}{1}
                {[|}{$\text{[}$}{1}
                {|]}{$\text{]}$}{1}
                {send}{$\tmkw{\uparrow}$}{1}
                {||}{$\tmkw{\mathbin{\vert\vert}}$}{1}                
}

